Scalable Ground Station Selection for Large LEO Constellations

Effective ground station selection is critical for low Earth orbiting (LEO) satellite constellations to minimize operational costs, maximize data downlink volume, and reduce communication gaps between access windows. Traditional ground station selection typically begins by choosing from a fixed set of locations offered by Ground Station-as-a-Service (GSaaS) providers, which helps reduce the problem scope to optimizing locations over existing infrastructure. However, finding a globally optimal solution for stations using existing mixed-integer programming methods quickly becomes intractable at scale, especially when considering multiple providers and large satellite constellations. To address this issue, we introduce a scalable, hierarchical framework that decomposes the global selection problem into single-satellite, short time-window subproblems. Optimal station choices from each subproblem are clustered to identify consistently high-value locations across all decomposed cases. Cluster-level sets are then matched back to the closest GSaaS candidate sites to produce a globally feasible solution. This approach enables scalable coordination while maintaining near-optimal performance. We evaluate our method's performance on synthetic Walker-Star test cases (1-10 satellites, 1-10 stations), achieving solutions within 95% of the global IP optimum for all test cases. Real-world evaluations on Capella Space (5 satellites), ICEYE (40), and Planet's Flock (96) show that while exact IP solutions fail to scale, our framework continues to deliver high-quality site selections.

==> Content/03.5_Results.tex <==
\section{Experiments}

We perform several evaluations of our scalable GSaaS placement framework, focusing on two main areas. First, we compare scalability and accuracy compared to exact integer programming formulations, where one-to-one comparisons can be made when the IP solver converges to the globally optimal solution. Second, we dive into the performance of our decomposition and clustering solution in realistic scenarios with higher complexity. The complexity arsies from both considering a larger number of candidate solutions $\mathcal{L}$ and the size of the satellite constellation $\mathcal{S}$ supported. These experiments are performed on the Capella Space, ICEYE, and Planet Labs' Flock constellations. In these scenarios, we demonstrate the effectiveness and scalability of our decomposition, clustering, and matching framework when the IP formulation alone fails.

Spacecraft dynamics are propagated using the SGP4 propagator \cite{vallado2006revisiting}. The simulation horizon $T_{sim}$ is set to 7 days, split into 1-day windows with 12-hour overlaps, resulting in 14 windows. The full optimization horizon $T_{opt}$ is set to 365 days for all cases. A $10^\circ$ minimum elevation mask is applied to all contact opportunities. Simulations were performed on a workstation with a 64-core 2.0 GHz AMD EPYC 7713 processor. Detailed design parameters for the main simulations are provided in \Cref{tab:design_parameters}.

\begin{table}[htbp]
\centering
\begin{tabular}{lr}
\toprule
Parameter & Value \\
\midrule
$t^{start}_{sim}$ & 2025-08-22 00:00:00 UTC \\
$t^{end}_{sim}$ & 2025-08-29 00:00:00 UTC \\
$t^{start}_{opt}$ & 2025-08-22 00:00:00 UTC \\
$t^{end}_{opt}$ & 2026-08-22 00:00:00 UTC \\
$C_{\text{dr}}$ & 1.2 Gbps \\
$\Delta t$ & 1 day \\
$T_{overlap}$ & 12 hours \\
$t_{\min}$ & 180 seconds \\
\bottomrule
\end{tabular}
\caption{Design parameters used for simulations.} 
\label{tab:design_parameters}
\vspace{-2em}
\end{table}

In our decomposed IP subproblems, we focus on two primary objectives: maximizing data downlink, and minimizing each satellite's maximum contact gap. These objectives capture the trade-offs inherent in designing ground station segments for satellite constellations, and we use the full IP objective function formation and constraints as described in \Cref{sec:problem_formulation}. Each IP subproblem is solved using Gurobi v11.0.3, and the resulting solutions are fed into our clustering and matching pipeline using the appropriate python \textsc{scikit-learn} and \textsc{scipy.optimize} libraries to select the final GSaaS locations. 



\subsection{Evaluating Decomposition Accuracy and Scalability}

We first evaluate our decomposition framework on small problem instances where an IP solver can still obtain exact solutions. For each test case, we generate new problem scenarios by varying the satellite constellation size $\lvert \mathcal{S} \rvert $ and the number of selected ground stations $n$. To do this, we construct a synthetic Walker-Star constellation with parameters in \Cref{tab:walker_star} to systematically vary constellation size and geometry. The number of orbital planes is varied from 1 to 10, producing constellations ranging from a single satellite to 10 satellites. We further increase problem complexity by varying the number of ground stations $n$ selected from our design candidate list $\mathcal{L}^D\subset\mathcal{L}$, which is restricted to the KSAT and Atlas Space networks. Optimizations with larger candidate site sets $\mathcal{L}$, and problems needing to select larger number of ground stations $n$ yield harder problems. Scenarios tested in this section are small enough to be solved using the full IP formulation. Using these smaller problems as a baseline, we then assess how well our decomposition, clustering, and matching framework approximates the optimal IP results as problems scale in size.



\begin{table}[htbp]
\centering
\begin{tabular}{lcr}
\toprule
Parameter & Value & Unit \\
\midrule
Altitude & 781 & km \\
Eccentricity & 0.001 & -- \\
Inclination & 86.4 & degrees \\
\# of Planes & $\{1,2,\dots,10\}$ & -- \\
\# of Sats per Plane & 1 & -- \\
\bottomrule
\end{tabular}
\caption{Walker-Star constellation parameters.} 
\label{tab:walker_star}
\vspace{-2em}
\end{table}


It is important to note that not all methods are directly comparable to the ground-truth IP solutions. The decomposed IP only solves smaller subproblems rather than the full problem, either over shorter simulation interval windows, and when applicable, smaller subsets of the constellation. Meanwhile, the DBSCAN-only clustering baseline identifies clusters of contacts but does not directly associate these clusters with final ground station locations, and thus does not enforce the original IP constraints. Only the DBSCAN + Hungarian matching and $k$-medoids approaches enforce constraints consistent with the full problem. The full list of methods is outlined in \Cref{tab:methods}.

\begin{table}[bp]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{p{2.6cm}p{1.1cm}p{3.6cm}}
\toprule
\textbf{Method} & \textbf{Directly compare to IP?} & \textbf{Description}\\
\midrule
IP-Optimal& $-$  & Exact integer programming solution (ground truth) \\
IP-Decomposed & No &IP formulation with temporal/spatial decomposition \\
DBSCAN Only & No & Clustering only (no assignment) \\
% DBSCAN + Greedy & Yes &DBSCAN clustering followed by greedy matching  \\
DBSCAN + Hungarian & Yes &DBSCAN clustering followed by Hungarian matching \\
$k$-Medoids &Yes & Joint clustering and matching \\
\bottomrule
\end{tabular}
\caption{Descriptions of methods evaluated, with comparability to the ground-truth IP solution.}
\label{tab:methods}
\end{table}


\begin{figure}[htbp]
  \centering
  % Left side: big figure

    \includegraphics[trim={1cm 1cm 0cm 1cm},scale = 0.35]{figures/IP_solution_MaxData_chunks=True.pdf}
    \caption{Optimal full-IP solution for total data downlinked as a function of selected $\#$ of ground stations and satellites in constellation. Serves as benchmark “true” solution, with all original constraints enforced.}
    \label{fig:IP_solmaxdata}
    \vspace{-2em}
\end{figure}

\begin{figure*}[htbp]
  \centering
  %   % Top full-width image
  % \includegraphics[trim={0cm 0cm 0cm 1cm}, width=0.7\linewidth]{figures/IP_solution_MaxData_chunks=True.pdf}
  % \caption{Optimal full-IP solution for total data downlinked as a function of selected \# of ground stations and satellites in constellation. Serves as benchmark “true” solution, with all original constraints enforced.}
  % \label{fig:IP_solmaxdata}
  % \vspace{-1em} % vertical space between top and bottom row
  % Left image (left-aligned)
  \begin{minipage}[t]{0.4\textwidth}
    \centering
    \includegraphics[scale=0.215]{figures/bulk_MaxData_chunks=False.pdf}
    \caption{Deviation in performance from optimum in maximum data downlink objective using scalable decomposition applied solely along the time dimension.}
    \label{fig:chunks_false_maxData}
  \end{minipage}%
  \hfill
  % Right image (right-aligned)
  \begin{minipage}[t]{0.4\textwidth}
    \centering
    \includegraphics[scale=0.215]{figures/bulk_MaxData_chunks=True.pdf}
    \caption{Deviation in performance from optimum in maximum data downlink objective using scalable decomposition applied along both time and satellite dimensions.}
    \label{fig:chunks_true_maxData}
  \end{minipage}
\end{figure*}

\subsubsection{Decompsition Levels} 
We first compare our methodology's performance on different levels of decomposition: temporal decomposition (using shorter time windows only) versus a combined approach of temporal and per-satellite decomposition. Experiments with maximum data downlink objective are shown in Figures \ref{fig:IP_solmaxdata}, \ref{fig:chunks_false_maxData}, and \ref{fig:chunks_true_maxData}, while those with minimum maximum-gap are shown in Figures \ref{fig:IP_solminmaxgap}, \ref{fig:chunks_False_minmaxgap}, and \ref{fig:chunks_true_minmaxgap}.

Starting with the maximum data objective, the full IP solution in \Cref{fig:IP_solmaxdata} provides the ground-truth optimal total downlink over $T_{opt}$ in petabytes (PB). In \Cref{fig:chunks_false_maxData,fig:chunks_true_maxData}, we plot the difference between this optimal solution and the best values achieved by each method across each test case. These difference heatmaps allow us to directly visualize where our methods match, improve upon, or fall short of the IP solution. Since we take the difference from the IP solution, any negative difference values (improved) is in blue, and any positive difference values (sub-optimal) are indicated in red. We similarly plot the ground-truth IP solution for the minimum maximum-gap objective in \Cref{fig:IP_solminmaxgap}, which displays maximum contact gap over all satellites in hours during over $T_{opt}$. In \Cref{fig:chunks_False_minmaxgap,fig:chunks_true_minmaxgap}, we similarly plot the difference between the optimal solution in \Cref{fig:IP_solminmaxgap} and the best values achieved by each method. 



\begin{figure}[htbp]
  \centering
  % Left side: big figure

    \includegraphics[trim={1cm 0cm 0cm 1cm},scale = 0.35]{figures/IP_solution_MinMaxGap_chunks=False.pdf}
    \caption{Optimal full IP solution for the smallest maximum gap in contact for all satellites as a function of selected $\#$ of ground stations and satellites in constellation. Serves as benchmark “true” solution, with all original constraints enforced.}
    \label{fig:IP_solminmaxgap}
    \vspace{-2em}
\end{figure}


\begin{table*}[htbp]
\centering
\begin{tabular}{@{}clcclccc@{}}
\toprule
\textbf{Position} & \textbf{Optimal IP} & \textbf{Longitude} & \textbf{Latitude} & \textbf{Clustering Methods\textsuperscript{*}} & \textbf{Longitude} & \textbf{Latitude} & \textbf{Distance (km)} \\
\midrule
1 & Long Beach & $-118.15$ & $33.82$ & Long Beach & $-118.15$ & $33.82$ & $0.0$ \\
2 & Singapore & $103.7$ & $1.32$ & Singapore & $103.7$ & $1.32$ & $0.0$ \\
3 & Svalbard & $15.41$ & $78.23$ & Svalbard & $15.41$ & $78.23$ & $0.0$ \\
4 & Troll & $2.53$ & $-72$ & Troll & $2.53$ & $-72$ & $0.0$ \\
5 & Tolhuin & $-67.12$ & $-54.51$ & Punta Arenas & $-70.87$ & $-52.94$ & $302.9$ \\
6 & Bangalore & $77.37$ & $12.9$ & Mauritius & $57.45$ & $-20.5$ & $4{,}289.9$ \\
\bottomrule
\end{tabular}
\caption{Comparison of ground station selections for the min-max gap objective with $n=6$ satellites. Both clustering/matching methods (DBSCAN+Hungarian and $k$-Medoids) selected identical stations. Maximum gap times: $0.9$ hours (Optimal IP), $1.24$ hours (clustering/matching).}
\label{tab:station_comparison}
\end{table*}
We emphasize that some methods are not strictly comparable to the ground-truth IP, since they do not enforce the same constraints. For example, the decomposed IP formulation for the maximum-data objective in \Cref{fig:chunks_false_maxData} partitions the problem by temporal windows, while \Cref{fig:chunks_true_maxData} decomposes even further by satellites. To compare these with the full IP, we scale the decomposed solutions to the full problem size (e.g., multiplying by the time horizon length and/or number of spacecraft in the constellation). This scaling produces solutions that approximate, but do not strictly satisfy the original IP constraints. For the minimum maximum-gap objective in \Cref{fig:chunks_False_minmaxgap,fig:chunks_true_minmaxgap}, scaling is unnecessary because the maximum gap time over each time window $T_{sim}^j\in\mathcal{T}$ is assumed to reflect the type of gap times found in both $T_{sim}$ and $T_{opt}$. Still, the reported values represent only the optimal outcomes from each time window $T_{sim}^j$ or each individual satellite $S$, not the global IP.

A similar caveat applies to the DBSCAN clustering baselines. Since cluster centers are not restricted to actual ground station locations in $\mathcal{L}^D$, DBSCAN-only solutions can occasionally outperform the true IP by placing “virtual” stations. Once cluster centers are mapped back to GSaaS sites (DBSCAN clustering with Hungarian matching or $k$-Medoids), the solutions become fully comparable to the ground truth.

In these final solutions with both clustering and matching performed, we observe generally strong performance with minimal deviation from the optimal IP site selections. For all cases with the maximum data downlink objective, solutions met up to $99\%$ of the optimal IP, and at least $94\%$ of cases with the minimium maximum-gap objective approached values of more than $95\%$ of the optimal solution. This strength can be partly attributed to the overperformance of the decomposed IP and DBSCAN-only baselines, which carries through to the matched solutions and only diminishes when enforcing the original problem constraints. Nevertheless, some test cases show underperformance, highlighted in red on the heatmaps, where matching back to feasible solutions proved overly restrictive. In particular, the $k$-Medoids method performs worse than DBSCAN clustering with Hungarian Matching for both objectives. This suggests that directly selecting cluster centers from GSaaS locations, as $k$-Medoids does, reduces flexibility and may lead to suboptimal coverage compared to approaches that first identify centroids and then map them back to feasible sites.



Comparing decomposition strategies for the maximum data downlink objective in \Cref{fig:chunks_false_maxData} (temporal only) and \Cref{fig:chunks_true_maxData} (temporal and satellite), we find that using both temporal and satellite-level decomposition yields solutions closer to the optimal IP. This improvement appears to stem from two factors. First, solving at the per-satellite level identifies locally optimal allocations tailored to each spacecraft, which can then be aggregated into stronger overall results. This effect is visible in the heatmaps of \Cref{fig:chunks_true_maxData}, which show more blue regions—indicating performance closer to, or even exceeding, the full IP—compared to the temporal-only case in \Cref{fig:chunks_false_maxData}. Second, satellite-level decomposition produces more data for the clustering pipeline, which could lead to richer solutions. In contrast, temporal-only decomposition may not yield sufficient diversity in candidate sites, limiting clustering performance when scaled to the full IP.



\begin{figure*}[htbp]
  \centering
  %   % Top full-width image
  % \includegraphics[trim={0cm 0cm 0cm 1cm}, width=0.7\linewidth]{figures/IP_solution_MaxData_chunks=True.pdf}
  % \caption{Optimal full-IP solution for total data downlinked as a function of selected \# of ground stations and satellites in constellation. Serves as benchmark “true” solution, with all original constraints enforced.}
  % \label{fig:IP_solmaxdata}
  % \vspace{-1em} % vertical space between top and bottom row
  % Left image (left-aligned)
  \begin{minipage}[t]{0.4\textwidth}
    \centering
    \includegraphics[scale=0.215]{figures/bulk_MinMaxGap_chunks=False.pdf}
    \caption{Deviation in performance from optimum in minimum maximum-gap objective using scalable decomposition applied solely along the time dimension.}
    \label{fig:chunks_False_minmaxgap}
  \end{minipage}%
  \hfill
  % Right image (right-aligned)
  \begin{minipage}[t]{0.4\textwidth}
    \centering
    \includegraphics[scale=0.215]{figures/bulk_MinMaxGap_chunks=True.pdf}
    \caption{Deviation in performance from optimum in minimum maximum-gap objective using scalable decomposition applied along both time and satellite dimensions.}
    \label{fig:chunks_true_minmaxgap}
  \end{minipage}
\end{figure*}


For the minimum maximum-gap objective, however, the trend reverses. Comparing \Cref{fig:chunks_False_minmaxgap} (temporal only) and \Cref{fig:chunks_true_minmaxgap} (temporal and satellite), we find that temporal-only decomposition achieves higher performance than the combined temporal-and-satellite strategy. Unlike the maximum data objective, the minimum maximum-gap metric depends on performance across the entire constellation rather than per-satellite allocations. Decomposing at the satellite level may lead to solutions that are overly specialized to individual spacecraft, but fail to capture constellation-wide coverage. When these satellite-level solutions are recombined and matched, the resulting performance can be slightly suboptimal relative to the original objective. However, we highlight that $92\%$ of test cases in the final DBSCAN with Hungarian matching selections are within $95\%$ of the optimal IP solution. Performance dips in our final solutions seem to be driven not by constellation size, but by the number of selected ground stations. Underperforming scenarios are concentrated along rows $4$, $6$, and $8$ in the heatmaps for the DBSCAN + Hungarian matching method. $k$-Medoids shows even stronger sensitivity, underperforming with larger ground station network sizes, at $n = 6, 7,$ and $8$.

Examining the selected stations of underperforming clustering scenarios of the minimum maximum-gap objective, we found that in most cases, the differences in coverage performance could be traced to a single ground station differing between the optimal and clustering solutions. As an illustrative example, we consider the minimum maximum-gap objective with $n=6$ stations selected from a Walker star constellation of size $\lvert S \rvert = 6$.  \Cref{tab:station_comparison} lists the ground station locations chosen by the optimal IP solution alongside those selected by our clustering and matching methods. In this case, both of our DBSCAN with Hungarian matching and $k$-Medoids methods produced identical station sets. The table highlights both the geographic coordinates and spatial proximity of the clustering-selected stations relative to the optimal solution. While almost all of the same station selections were made as the optimal IP, one single difference in station choice noticeably reduced performance. In this example, the maximum gap time in contact across the constellation is $0.9$ hours for the optimal IP solution, compared to $1.24$ hours for the clustering and matching methods. The fact that such differences stem from a single station suggests that modest, targeted refinements, or individual station swaps for further post-processing could further close performance gaps.




\begin{figure}[htbp]
    \centering
    \includegraphics[trim={0cm 24cm 0cm 0cm},clip,scale=0.3]{figures/ALL_bulk_MaxData_chunks=True.pdf}
    \caption{Deviation in solution performance from optimal full-IP solution for the maximum data downlink scenario, when expanding the initial clustering solutions to the full $\mathcal{L}$ ground station candidate site list.}
    \label{fig:all_expansion}
    \vspace{-1em}
\end{figure}

\subsubsection{Expanding Candidate Ground Station Locations}
We next evaluate the performance of our clustering–matching methods when expanding the candidate ground station set from the design GSaaS subset $\mathcal{L}^D$ (KSAT, Atlas Space) to the full list of candidate sites $\mathcal{L}$ (Atlas Space Operations, AWS Ground Station, Azure Orbital, KSAT, Leaf Space, and Viasat). For the maximum-data downlink objective, we can benchmark directly against the optimal IP solution, as shown in \Cref{fig:all_expansion}. In this setting, the clustering-based methods nearly match the optimal solutions, demonstrating that if the restricted set $\mathcal{L}^D$ is sufficiently diverse, the clustering and matching framework can extrapolate effectively to select near-optimal ground station locations in the full candidate list $\mathcal{L}$. We observe slight degradation for larger selections, specifically $n=9$ or $10$, but the suboptimality remains modest, still approaching $99\%$ of the original solution. For the min–max gap objective, we are unable to provide direct comparisons in this expanded setting, since the full IP solutions fail to converge reliably.


\subsection{Realistic Scenarios}

We next evaluate our framework on more realistic Earth observation constellations, where the number of satellites, ground station candidates, and overall problem complexity is substantially larger than in the controlled Walker star experiments. In this setting, we test our DBSCAN clustering with Hungarian matching method on three representative operators: Capella Space, ICEYE, and Planet Labs' Flocks, with constellation characteristics summarized in \Cref{tab:EO_Operators}. Once again for the decomposition step, time windows are split into 1-day windows with 12-hour overlaps, and the candidate ground station list $\mathcal{L}^D$ is restricted to the KSAT and Atlas Space GSaaS networks. However, after clustering is performed on these subproblems, we expand back in the matching phase the candidate ground station list to the full list of $\mathcal{L}$, exemplifying the scalability of our approach. We consider both the maximum-data downlink and minimum maximum-gap objectives. Where the full IP solution is computationally tractable, we use it as a benchmark; otherwise, we compare the degredation in solution answers from the initial subproblem decomposition to the final matching step to understand how our method performs at each stage of the scalable decomposition process.

\begin{table}[htbp!]
\centering
\begin{tabular}{lccc}
\toprule
Constellation & \# Sats & Altitude (km) & Inclination \\
\midrule
Capella Space & 5 & 525--575 & $45^\circ$, $53^\circ$, $97^\circ$ \\
ICEYE & 34 & 560--580 & $97^\circ$ \\
Planet Flocks & 93 & 500 & $97^\circ$ \\
\bottomrule
\end{tabular}
\caption{Earth Observation Satellite Constellations.} 
\label{tab:EO_Operators}
\end{table}




\begin{table*}[htbp] 
\centering
\begin{tabular}{lcccccccccrr}
\toprule
           & \multicolumn{3}{c}{Decomposition} 
           & \multicolumn{3}{c}{DBSCAN Clustering} 
           & \multicolumn{3}{c}{\textbf{Final Hungarian Match}} 
           &  \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
           % & Data Downlink & Maximum Gap 
           % & Data downlink & Maximum Gap 
           % & Data downlink & Maximum Gap 
           % & \\
           Constellation & Min  & Mean & Max
           & Min  & Mean & Max
           & Min  & Mean & Max
           & Optimal & Solution $\Delta$\\
\midrule
Capella Space      &   3.21& 6.10&  6.85&   
4.84& 5.03& 5.06&  4.99& 5.05&  \textbf{5.07}& \textbf{5.23} &1.78 \\
ICEYE      &  12.77&  44.05  &  55.97 & 38.89  &  41.95   &  42.99 & 34.88  &  40.81   &  \textbf{43.03 } & \textbf{43.04} &12.84\\
Flock      &  40.72&  96.34  &  112.23 & 85.80  &  93.86   &  96.33 & 90.32  &  94.54   &  \textbf{96.43 } & \textbf{96.45}&15.8\\
\bottomrule
\end{tabular}
\caption{Performance of scalable decomposition and clustering methods at each stage in comparison to optimal IP formulation. The approach uses 1-day time windows with per-satellite decomposition, DBSCAN clustering, and Hungarian matching for final GSaaS solutions. Optimizing for maximum data downlink objective, values listed in PB over $T_{opt}$.
Solution $\Delta$ represents the difference between maximum per-satellite decomposed solutions and final Hungarian matching solutions.}
\label{tab:RealData}
\end{table*}



\begin{table*}[htbp] 
\centering
\begin{tabular}{lcccccccccrr}
\toprule
           & \multicolumn{3}{c}{Decomposition} 
           & \multicolumn{3}{c}{DBSCAN Clustering} 
           & \multicolumn{3}{c}{\textbf{Final Hungarian Match}} 
           &  \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
           % & Data Downlink & Maximum Gap 
           % & Data downlink & Maximum Gap 
           % & Data downlink & Maximum Gap 
           % & \\
           Constellation & Min  & Mean & Max
           & Min  & Mean & Max
           & Min  & Mean & Max
           & Optimal 
           & Solution $\Delta$
           \\
\midrule
Capella Space      &   0.61& 0.85&  1.14&   
2.33& 2.64& 3.56&  \textbf{2.31}& 2.73&  3.56& \textbf{1.42} & 1.17\\
ICEYE      &  0.53 &  0.88  &  1.31 & 2.43  &  3.31   &  4.50 & \textbf{2.46}  &  3.52   &  4.50 & \textbf{-} & 1.15\\
Flock      &  0.77 &  0.89 &  1.13& 1.44 &  1.55  &  1.58 & \textbf{1.44}  &  1.65   &  1.66 & \textbf{-} &0.31\\
\bottomrule
\end{tabular}
\caption{Performance of scalable decomposition and clustering methods compared to optimal IP formulation. The approach uses 1-day time windows with per-satellite decomposition, DBSCAN clustering, and Hungarian matching for final GSaaS solutions. All values optimize for minimum maximum-gap between contacts (hours over $T_{opt}$). Solution $\Delta$ represents the difference between minimum per-satellite decomposed solutions and final Hungarian matching solutions. Optimal solutions from IP solvers failed to converge for ICEYE and Planet Labs' FLOCK constellations.}
\label{tab:RealGap}
\end{table*}

For the maximum data downlink objective, we were able to directly compare our results to the optimal solutions obtained from the IP solver, allowing us to evaluate how each step of our scalable framework performs with these realistic constellation scenarios. Evaluations of the subproblems within our framework is outlined at three stages: (1) the decomposition results, (2) DBSCAN clustering of the decomposed solutions, and (3) the final Hungarian matching that maps cluster centroids to actual GSaaS station locations. It is important to note that the decomposition and clustering results are not perfectly comparable to the optimal solution, since we normalize decomposition values (by constellation size and time window length), and clustering solutions are generated before enforcing the final station-location constraints. The full numerical results are presented in \Cref{tab:RealData}.

Because performance varies across satellites, decompositions, and clustering parameters, we report ranges (minimum, mean, maximum) for each method. In decomposition, the spread reflects different satellite splits; in clustering, it depends on the choice of neighborhood DBSCAN distance thresholds $\varepsilon$, which ranged from $\{5,10,15,20,25,30,35,40\}$; and the final Hungarian match inherits the variability from clustering. Among these, we are primarily interested in the maximum values, since they represent the “best-case” achievable solutions that should be closest to optimal.

Overall, we find that solution quality decreases when moving from decomposition to clustering—an expected result, since decomposition represents an upper bound (best-case across satellites and time splits), while clustering introduces variability and weaker minimum solutions. Interestingly, the final Hungarian match slightly improves upon the clustering stage in several cases. This suggests that mapping cluster centroids to real GSaaS station locations does not degrade performance as much as expected, and may even benefit from the spatial distribution of actual stations. When compared to the optimal IP solutions, the final matched results are extremely close across most constellations. The main exception is Capella Space, which shows a modest performance gap. This is likely due to its distinct orbital regime with different altitudes and inclination angles for its spacecraft. However, even in this case, the performance of our scalable site selection method remains within a reasonable bound near the optimal IP solution. The approximate value after matching is at 5.07 PB, about 3.06\% lower than the optimal 5.23 PB over $T_{opt}$.



Now, examining the results for the minimum maximum-gap objective in \Cref{tab:RealGap}, we observe trends that differ from the maximum data downlink case. For this objective, the minimum values are the most meaningful, since the goal is to reduce the largest gap between consecutive satellite contacts. The exception is the decomposition-per-satellite metric, where by the objective's definition we select the maximum to represent the maximum gap found in communications across the constellation.

Transitioning from decomposition to DBSCAN clustering introduces a noticeable increase in the maximum gap for both Capella Space and ICEYE constellations. Surprisingly, the largest constellation, FLOCK, exhibits a smaller increase in maximum gap. This is likely due to its satellites having similar orbits, whereas Capella Space and ICEYE have varied orbital altitudes. Capella Space even has differences in inclination angles for its small constellation, explaining why its loss in solution quality is comparable to ICEYE, despite ICEYE having almost eight times more satellites.

Only the Capella Space constellation, with 5 satellites, could be solved using the full IP formulation, highlighting the difficulty of scaling IP solvers for larger constellations and full candidate GSaaS lists for consideration. For Capella Space, comparing the optimal solution (1.42 hours) to the final Hungarian-matched solution (2.31 hours) shows a difference from the true optimum. However, considering the length of the entire optimization window, the approximate solution still provides a good start. For ICEYE and Flock, the full optimal solution is intractable, but the final solutions remain close to the decomposition step considering the size of each constellation. For example, Flock's final solution has a maximum gap of 1.44 hours versus 1.13 hours from the satellite-specific decomposition, indicating only a modest loss in solution quality despite expanding the selected sites to the entire 96 satellite constellation.

These results suggest that our decomposition-clustering-matching framework performs especially well for large constellations with similar orbital regimes. Despite ICEYE having eight times more satellites than Capella Space, the solution $\Delta$ remains comparable, indicating this method provides an effective starting point for minimizing maximum gap times in large-scale scenarios.

